Misquoted No More: Securely Extracting F* Programs with IO

Shallow embeddings that use monads to represent effects are popular in proof-oriented languages because they are convenient for formal verification. Once shallowly embedded programs are verified, they are often extracted to mainstream languages like OCaml or C and linked into larger codebases. The extraction process is not fully verified because it often involves quotation -- turning the shallowly embedded program into a deeply embedded one -- and verifying quotation remains a major open challenge. Instead, some prior work obtains formal correctness guarantees using translation validation to certify individual extraction results. We build on this idea, but limit the use of translation validation to a first extraction step that we call relational quotation and that uses a metaprogram to construct a typing derivation for the given shallowly embedded program. This metaprogram is simple, since the typing derivation follows the structure of the original program. Once we validate that the typing derivation is valid for the original program, we pass it to a verified syntax-generation function that produces code guaranteed to be semantically related to the original program. We apply this general idea to build SEIO*, a framework for extracting shallowly embedded F* programs with IO and refinement types to a deeply embedded simply typed lambda-calculus while providing formal secure compilation guarantees. Using two cross-language logical relations, we devise a machine-checked proof in F* that SEIO* guarantees Robust Relational Hyperproperty Preservation (RrHP), a very strong secure compilation criterion that implies full abstraction as well as preservation of trace properties and hyperproperties against arbitrary linked adversarial code. This goes beyond the state of the art in verified and certifying extraction, which so far has focused on correctness rather than security.

==> lstfstar.tex <==
\newcommand\function{\sffamily\maybecolor{dkblue}function}

\makeatletter
\lstdefinelanguage{fstar}{%
  basicstyle=\small,
  morekeywords=[1]{type,and,val,fun,let,in,ref,uref,mref,try,if,then,else,match,with,open,as,module,rec,begin,end,assume,private,when,forall,assert,by_tactic,logic,array,pattern,effect,requires,ensures,decreases,modifies, abstract,total, reifiable, reflectable, new_effect, effect_actions, noeq, sub_effect, by, synth,splice,class,instance},
  morekeywords=[2]{WP, Post, Pre, Pure , PURE, DIV, Dv, STATE, EXN, ALL,
                   TotST, M, GHOST, Ghost, GTot, Lemma, Tot, Div, DIV,
                    Memo, READER, STATE_m, Effect, STEXN, RANDOM, ST, 
                    St, MST, MSTATE, MSTFlag, S_MST, MSTExn, TAC, Tac,
                     TacH, Type,
                     EVar, ELam, EFileDescr, EString, ERead, EWrite, 
                     EOpen, EClose, EUnit, Etrue, Efalse, EIf, EPair, 
                     EFst, ESnd, ECase, EInl, EInr, EApp, EvOpen, EvRead,
                     EvClose, EvWrite, ELambda, EFailedValidation,EZero, ESucc, ENRec,
                     Qfalse,QAxiom,QWeaken,QApp,QLambda,QInl,QCase,QInr,QInl, Qtrue, QStringLit,
                     QIfIO,QAppIO,QLambdaIO,QFailedValidation,Qtt,QReturn,QBind,QRead,QWrite,QClose,
                     QOpenfile,QCaseIO,EvOpenfile,QIf,QMkpair,QFst,QSnd,QZero,QSucc,QNRec,QRef},

  morekeywords=[3]{},
  morekeywords=[4]{},
  morekeywords=[5]{solve},
  morestring=[b]",
  sensitive=true,%

  numbersep=4pt,
%  numbers=left,
  columns=[l]fullflexible,
  texcl=true,
  mathescape=true,
%  xleftmargin=10pt,
  identifierstyle={\sffamily},
  keywordstyle=[1]{\sffamily\maybecolor{dkblue}},
  keywordstyle=[2]{\sffamily\maybecolor{dkblue}},
  keywordstyle=[3]{\maybecolor{dkred}},
  keywordstyle=[4]{\rmfamily\itshape},
  keywordstyle=[5]{\bf\sffamily},
% Here is the range marker stuff
  rangeprefix=(*---\ ,
  includerangemarker=false,
  stringstyle=\ttfamily,
  %lineskip=-2pt,
  showspaces=false,
  morecomment=[n]{(*}{*)},
  commentstyle={\itshape\maybecolor{dkred}},
  literate={->}{$\rightarrow\,$}{1}
           {typing_oval}{\sffamily typing}{1}
           {typing_oprod}{\sffamily typing$_{\text{io}}$}{1}
           {typing_oval\ }{\sffamily typing }{1}
           {typing_oprod\ }{\sffamily typing$_{\text{io}}$ }{1}
           {tyG}{$\Gamma$}{1}
           {tyG\ }{$\Gamma$ }{1}
           {fsG}{$\gamma$}{1}
           {fsG\ }{$\gamma$ }{1}
           {fsGs}{$\gamma_\star$}{1}
           {fsGs\ }{$\gamma_\star$ }{1}
           {eGs}{$\gamma_\lambda$}{1}
           {eGs\ }{$\gamma_\lambda$ }{1}
           {preG}{$\phi$}{1}
           {∋}{$\ni$}{1}
           {∋\ }{$\ni$ }{1}
           {∈}{$\in$}{1}
           {∈\ }{$\in$ }{1}
           {⊇}{$\supseteq$}{1}
           {⊇\ }{$\supseteq$ }{1}
           {⊆}{$\subseteq$}{1}
           {⊆\ }{$\subseteq$ }{1}
           {⫄}{$\supseteq_{\text{io}}$}{1}
           {⫄\ }{$\supseteq_{\text{io}}$ }{1}
           {⫃}{$\subseteq_{\text{io}}$}{1}
           {⫃\ }{$\subseteq_{\text{io}}$ }{1}
           {⊐}{$\sqsupseteq$}{1}
           {⊐\ }{$\sqsupseteq$ }{1}
           {⊒}{$\sqsupseteq_{\text{io}}$}{1}
           {⊒\ }{$\sqsupseteq_{\text{io}}$ }{1}
           {e_beh}{\sffamily beh$_\lambda$}{1}
           {fs_beh}{\sffamily beh$_\star$}{1}
           {e_beh\ }{\sffamily beh$_\lambda$ }{1}
           {fs_beh\ }{\sffamily beh$_\star$ }{1}
           % fs_-prefixed IO* identifiers: drop the prefix, add a subscript star
           % (primed names stack the prime over the star). IMPORTANT: listings
           % literate gives the LAST matching key precedence (not the longest),
           % so each base name must be listed BEFORE its longer forms -- e.g.
           % fs_r before fs_r_f, fs_x before fs_x'. The "\ " variants preserve a
           % trailing space, which the replacement would otherwise swallow.
           {fs_k}{\sffamily k$_\star$}{1}
           {fs_k\ }{\sffamily k$_\star$ }{1}
           {fs_m}{\sffamily m$_\star$}{1}
           {fs_m\ }{\sffamily m$_\star$ }{1}
           {fs_oe}{\sffamily oe$_\star$}{1}
           {fs_oe\ }{\sffamily oe$_\star$ }{1}
           {fs_arg}{\sffamily arg$_\star$}{1}
           {fs_arg\ }{\sffamily arg$_\star$ }{1}
           {fs_val}{\sffamily val$_\star$}{1}
           {fs_val\ }{\sffamily val$_\star$ }{1}
           {fs_e}{\sffamily e$_\star$}{1}
           {fs_e\ }{\sffamily e$_\star$ }{1}
           {fs_e'}{\sffamily e$^{\smash{\raisebox{-0.83ex}{\mbox{\sffamily\textquotesingle}}}}_{\smash{\raisebox{0.25ex}{$\scriptstyle\star$}}}$}{1}
           {fs_e'\ }{\sffamily e$^{\smash{\raisebox{-0.83ex}{\mbox{\sffamily\textquotesingle}}}}_{\smash{\raisebox{0.25ex}{$\scriptstyle\star$}}}$ }{1}
           {fs_f}{\sffamily f$_\star$}{1}
           {fs_f\ }{\sffamily f$_\star$ }{1}
           {fs_f'}{\sffamily f$^{\smash{\raisebox{-0.83ex}{\mbox{\sffamily\textquotesingle}}}}_{\smash{\raisebox{0.25ex}{$\scriptstyle\star$}}}$}{1}
           {fs_f'\ }{\sffamily f$^{\smash{\raisebox{-0.83ex}{\mbox{\sffamily\textquotesingle}}}}_{\smash{\raisebox{0.25ex}{$\scriptstyle\star$}}}$ }{1}
           {fs_v}{\sffamily v$_\star$}{1}
           {fs_v\ }{\sffamily v$_\star$ }{1}
           {fs_v'}{\sffamily v$^{\smash{\raisebox{-0.83ex}{\mbox{\sffamily\textquotesingle}}}}_{\smash{\raisebox{0.25ex}{$\scriptstyle\star$}}}$}{1}
           {fs_v'\ }{\sffamily v$^{\smash{\raisebox{-0.83ex}{\mbox{\sffamily\textquotesingle}}}}_{\smash{\raisebox{0.25ex}{$\scriptstyle\star$}}}$ }{1}
           {fs_m'}{\sffamily m$^{\smash{\raisebox{-0.83ex}{\mbox{\sffamily\textquotesingle}}}}_{\smash{\raisebox{0.25ex}{$\scriptstyle\star$}}}$}{1}
           {fs_m'\ }{\sffamily m$^{\smash{\raisebox{-0.83ex}{\mbox{\sffamily\textquotesingle}}}}_{\smash{\raisebox{0.25ex}{$\scriptstyle\star$}}}$ }{1}
           {fs_k'}{\sffamily k$^{\smash{\raisebox{-0.83ex}{\mbox{\sffamily\textquotesingle}}}}_{\smash{\raisebox{0.25ex}{$\scriptstyle\star$}}}$}{1}
           {fs_k'\ }{\sffamily k$^{\smash{\raisebox{-0.83ex}{\mbox{\sffamily\textquotesingle}}}}_{\smash{\raisebox{0.25ex}{$\scriptstyle\star$}}}$ }{1}
           {fs_x}{\sffamily x$_\star$}{1}
           {fs_x\ }{\sffamily x$_\star$ }{1}
           {fs_x'}{\sffamily x$^{\smash{\raisebox{-0.83ex}{\mbox{\sffamily\textquotesingle}}}}_{\smash{\raisebox{0.25ex}{$\scriptstyle\star$}}}$}{1}
           {fs_x'\ }{\sffamily x$^{\smash{\raisebox{-0.83ex}{\mbox{\sffamily\textquotesingle}}}}_{\smash{\raisebox{0.25ex}{$\scriptstyle\star$}}}$ }{1}
           {valid_contains}{$\overset{\ni}{\approx}$}{1}
           {valid_contains\ }{$\overset{\ni}{\approx}$ }{1}
           {valid_superset_val\ }{$\overset{\supseteq}{\approx}$ }{1}
           {valid_superset_prod\ }{$\overset{\supseteq_{\text{io}}}{\approx}$ }{1}
           {valid_member_of}{$\overset{\in}{\approx}$}{1}
           {valid_member_of\ }{$\overset{\in}{\approx}$ }{1}
           {valid_subset_val\ }{$\overset{\subseteq}{\approx}$ }{1}
           {valid_subset_prod\ }{$\overset{\subseteq_{\text{io}}}{\approx}$ }{1}
           {Type0}{{\sffamily\maybecolor{dkblue} Type}$_0$}{1}
           {True}{$\top$}{1}
           {False}{$\bot$}{1}
           {exists}{$\exists$}{1}
           {forall}{$\forall$}{1}
           {fun}{$\lambda$}{1}
           {~}{$\neg$}{1}    
           {∽}{$\sim$}{1}
           {≍}{$\asymp$}{1}       
           {~>}{$\leadsto$}{1}
           {`}{\`{}}{1}
           {'a}{$\alpha$}{1}
           {'b}{$\beta$}{1}
           {'c}{$\gamma$}{1}
           {`star`}{$\ast\,$}{1}           
           {-*}{$\mbox{\endash}\ast\,$}{1}                      
           {Gamma}{$\Gamma\,$}{1}
           {theta}{$\theta\,$}{1}
           {_0}{$_0$}{1}
           {_1}{$_1$}{1}
           {_2}{$_2$}{1}
           {_3}{$_3$}{1}
           {_4}{$_4$}{1}
           {/\\}{$\wedge\;$}{1}
           {\\/}{$\vee\;$}{1}
           {>=}{$\geq\ $}{2}
           {<=}{$\leq\ $}{2}
           {[=}{$\mathrel{\sqsubseteq}$}{2}
           {<==>}{$\Longleftrightarrow \ $}{3}
           {==>}{$\Longrightarrow \ $}{3}
           {|->}{$\mapsto \ $}{3}
           {<>}{$\neq$}{1}
           {--}{-}{1}   % Added due to         - not displaying properly.  Weird. ... but may make arrows look bad  {...}{$\ldots$}{3}
           {<<}{$\prec\ $}{1}
           {alpha}{{$\alpha\ $}}{1}
           {vdots}{{\bf{\raisebox{-1pt}[0pt][0pt]{$\vdots$}}}}{1}
           {^S}{{{\raisebox{-1pt}[0pt][0pt]{${}^S$}}}}{1}
           {^T}{{{\raisebox{-1pt}[0pt][0pt]{${}^T$}}}}{1}
           {PTIT}{{{\raisebox{-1pt}[0pt][0pt]{${}^T$}}}}{1}
           {ISD}{{{\raisebox{-3pt}[0pt][0pt]{${}_{I^S\downarrow}$}}}}{1}
           {EOF}{{\ }}{1}
           ,
  breaklines=false}
\makeatother


==> texdirectives.tex <==
\draftfalse\anonfalse

